Tight Bounds for MIS in Multichannel Radio Networks

Daum et al. [PODC'13] presented an algorithm that computes a maximal independent set (MIS) within $O(\log^2 n/F+\log n \mathrm{polyloglog} n)$ rounds in an $n$-node multichannel radio network with $F$ communication channels. The paper uses a multichannel variant of the standard graph-based radio network model without collision detection and it assumes that the network graph is a polynomially bounded independence graph (BIG), a natural combinatorial generalization of well-known geographic families. The upper bound of that paper is known to be optimal up to a polyloglog factor. In this paper, we adapt algorithm and analysis to improve the result in two ways. Mainly, we get rid of the polyloglog factor in the runtime and we thus obtain an asymptotically optimal multichannel radio network MIS algorithm. In addition, our new analysis allows to generalize the class of graphs from those with polynomially bounded local independence to graphs where the local independence is bounded by an arbitrary function of the neighborhood radius.

==> hf-analysis/lemma-heraldwcpgoodherald.tex <==

% \sebastian{notes for later: we also don't want herald candidates in a broader neighborhood. leaders and heralds, however, must be allowed to exist nearby. Thus, statement needs to be extended such that fabian's proof does fit. maybe we can disallow leaders/heralds in $u$'s $2$-neighborhood, but i fear that's too tough.}
% \sebastian{this really needs to be checked for errors; as it must hold for any kind of scenario in which $u$ and $v$ are active in round $t$. e.g., this is wrong if they are neighboring another good leader-herald pair but manage to bypass their really low activity levels. i.e., we need to add a ton of additional requirements.}
% \sebastian{note for next adjustment: hinder that nodes communicate on channel $\lambda$ also in a larger radius around $u$.}


% \begin{proof}
\ifthenelse{\boolean{swapheraldclaim}}{}{
The proof for the lemma is not straightforward. We consider the two cases of $\Activity(u)>2$ and $\Activity(u) \leq 2$ and for those we establish claims about the probabilities for $u$ to become a herald in general and a good herald in particular before we provide the proof for Lemma \ref{lemma:heraldwcpgoodherald}.
Recall that $\Activity_\Astate(u)$ is the activity mass of all active nodes in $N^1(u)$ and that $\AAC(u)$ is the mass of those in $N(u)$, i.e., $\AAC(u)=\Activity_\Astate(u)-\activity(u)$.     


% \sebastian{the proof actually shows ``only'' $\Pr(D^u)=\Omega(\\Pr(B^u))$, but that suffices.... change statements.}

\begin{myclaim}
  \label{claim:heraldbounds}
  Let $r$ be a round in which node $u$ is in state \Astate and $N_\Astate(u) \neq \emptyset$.
  Let $B^u$ be the event that at the end of round $r$, $u$ moves to state
  $\Hstate'$ due to receiving a message from some node $v \in
  N_\Astate(u)$ on some channel $\Achannel_{\bar{\lambda}}$. Further, let $D^u\subseteq B^u$ be the event that
  $B^u$ holds and in addition no other node $v' \in N^3(v)\setminus\set{u}$
  receives any message on channel $\Achannel_{\bar{\lambda}}$ in round $r$. 
  It holds that
  \begin{eqnarray}
    \label{eq:claimequationsupper}
    \Pr(B^u) &=&
    \begin{cases}
      \bigO\brackets{\pi_\ell \frac{\activity(u)}{\AAC(u)}} & \AAC(u) > 2 \\
      \bigO\brackets{\pi_\ell \activity(u) \AAC(u)} & \AAC(u) \leq 2      
    \end{cases},
    \\
    \label{eq:claimequationslower}
    \Pr(D^u) &=&
    \begin{cases}
      \Omega\brackets{\pi_\ell \frac{\activity(u)}{\AAC(u)}} & \AAC(u) > 2 \\
      \Omega\brackets{\pi_\ell \activity(u) \AAC(u)} & \AAC(u) \leq 2      
    \end{cases}.
  \end{eqnarray}
\end{myclaim}
}

\begin{proof}
  In the calculations below we make use of the following inequalities.
  \begin{eqnarray}
    \label{eq:basic1}
    1-\pi_\ell &\geq& 0.9 \\
    \label{eq:basic2}
    1-x &\leq& e^{-x}, \quad \forall x \\
    \label{eq:basic3}
    1-x &\geq& e^{-2x}, \quad \forall x \in [0,1/2] \\
    \label{eq:basic4}
    \prod_{w \in A\setminus B} f(w) &\leq& F^{|B|} \prod_{w \in A} f(w), \quad \mbox{if } f(w) \geq F^{-1}
  \end{eqnarray}

  If $\AAC(u) > 2$, for simplicity, we assume that $\log \AAC(u)$ is a positive integer. It becomes clear from the proof that for non-integer values 
  % $\log \AAC(u) \in (\lfloor \log \AAC(u)\rfloor, \lceil\log\AAC(u)\rceil)$ 
  an adaption is straightforward, but hard to read.

  We let $B^{u,v}_i$ be the event that an \emph{active} node $u$ receives a message from an \emph{active} node $v$ on channel $\Achannel_i$, i.e., $u$ listens and $v$ broadcasts on $\Achannel_i$, while no other node $w \in (N_\Astate(u))\setminus\set{v}$ broadcasts on $\Achannel_i$. For different $v$ these events are disjoint, and we can define $B^u_i := \bigcup_{v \in N_\Astate(u)} B^{u,v}_i$ and we see that $B^u = \bigcup_{i=1}^{n_\Achannel} B^u_i$.

  % More restrictive are the analogously defined events $D^{u,v}_i$, $D^u_i$, in which we also require that no node $x \in N(v)\setminus\set{u}$ receives $v$'s message. In that case, $D^u=\bigcup_{i=1}^{n_\Achannel} D^u_i$ is the event that nodes $u$ and $v$ engage in the handshake protocol next round, without other herald candidates trying to do this with $v$ as well.

  More restrictive are the analogously defined events $D^{u,v}_i$, $D^u_i$, in which we also require that no node $x \in N^3(v)\setminus\set{u}$ receives a message on channel $i$. In that case, $D^u=\bigcup_{i=1}^{n_\Achannel} D^u_i$ is the event that nodes $u$ and $v$ engage in the handshake protocol in the round after they met on some channel $\Achannel_{\bar{\lambda}}$, without other nodes nearby having received something on that same channel. In particular, no other herald candidates try to engage with $v$ in the handshake protocol.

  % \sebastian{the upper bounds should be untouched by the change to the definition of $D^u$.}

  % Note that $H_u = B^u$ and $\hat{H}_u \subset D^u$.


  % for upper bounds we can calculate in a rather rough way, but we have to upper bound over all channels
  % for lower bounds we just have to look at \Achannel_1 or \Achannel_\lambda, but we have to exclude the possibility of other receivers around $v$
  \paraclose{Upper Bounds}

  Let $q_i^w$ be the probability that node $w$ does broadcast on channel $\Achannel_i$, i.e., $q_i^w = (1-\pi_\ell)\activity(w)2^{-i} \leq 1/4$, and accordingly $\bar{q}^w_i := 1-q^w_\lambda \geq 3/4$ is the probability that $w$ does not broadcast on channel $\Achannel_i$. We denote with $p_i^w$ the probability that $w$ listens on channel $\Achannel_i$. 

  \begin{equation*}
    \begin{split}
      \label{eq:BuviUB}
      \Pr(B^{u,v}_i)
      & = p_i^u q_i^v \prod_{w \in N_\Astate(u)\setminus\set{v}} \bar{q}_i^w 
      = \pi_\ell \activity(u) 2^{-i}(1-\pi_\ell) \activity(v) 2^{-i} \prod_{w \in N_\Astate(u)\setminus\set{v}} \bigbrackets{ 1-(1-\pi_\ell)\activity(w)2^{-i} } \\
      & \stackrel{(\ref{eq:basic2}),(\ref{eq:basic4})}{\leq} 
      \pi_\ell \activity(u)\activity(v)2^{-2i}
      % \underbrace{\frac{1}{1-(1-\pi_\ell)\activity(v)2^{-i}}}_{\leq 2} e^{-\frac{1}{2}\AAC(u)2^{-i}}
      \frac{4}{3} e^{-\frac{1}{2}\AAC(u)2^{-i}}
    \end{split}
  \end{equation*}

  \begin{equation}
    \label{eq:BuiUB}
    \Pr(B^u_i) \leq \pi_\ell \activity(u) \AAC(u) 2^{-2i+1} e^{-\AAC(u)2^{-i-1}} = 8\pi_\ell \frac{\activity(u)}{\AAC(u)} (\AAC(u) 2^{-i-1})^2 e^{-\AAC(u)2^{-i-1}} =: C^u_i
    % \leq \pi_\ell \activity(u) \Activity_\Astate(u) 2^{-2i+2} e^{-\Activity_\Astate(u)2^{-i-1}}
  \end{equation}

  Consider the case $\AAC(u) >2$. 
  % and for simplicity let $\lambda:= \log \AAC(u)$ be an integer. 
  For any $\zeta>0$ it holds that $\zeta^2e^{-\zeta}=\bigO(1)$, and by using $\zeta=\AAC(u)2^{-i}$ and we get that for any fixed $i$
  \begin{equation}
    \label{eq:CuiUB}
    C^u_i = \bigO\Big(\pi_\ell \frac{\activity(u)}{\AAC(u)}\Big) \quad \mbox{and} \quad C^u_i=\Theta(C^u_{i+1})
  \end{equation}
  Furthermore, with $\lambda := \log \AAC(u)$:
  \begin{align*}
    \frac{C_{i+1}^u}{C_i^u} &= \frac{1}{4}e^{\frac{1}{4}\AAC(u)2^{-i}} < \frac{1}{2} & \forall i &\geq \lambda\\
    \frac{C_{i}^u}{C_{i+1}^u} &=  4e^{-\frac{1}{4}\AAC(u)2^{-i}} < \frac{1}{2} & \forall i &\leq \lambda -4
  \end{align*}
  Thus, the sum of all $C^u_i$ with $i$ larger than $\lambda$ can be upper bounded by $C^u_\lambda$ using the geometric series, and, if $\lambda > 4$, all $i \leq \lambda-4$ can be upper bounded by $C^u_{\lambda-4}$. However, due to (\ref{eq:CuiUB}), $C^u_{\lambda-4}+ \dots + C^u_\lambda$ is in $\bigO(C^u_\lambda)=\bigO\bb{\pi_\ell \frac{\activity(u)}{\AAC(u)}}$.
  In total we get that
  % \begin{equation*}
  %   \label{eq:BuUB}
  $
  \Pr(B^u) = \bigO\bb{\pi_\ell \frac{\activity(u)}{\AAC(u)}}.
  $
  % \end{equation*}

  Now consider the case $\AAC(u) \leq 2$. 
  % and let $\lambda :=1$. 
  In (\ref{eq:BuiUB}) we upper bound $e^{-\AAC(u)2^{-i-1}}$ by $1$ and get
  \begin{equation*}
    \Pr(B^u_i) \leq \pi_\ell \activity(u) \AAC(u) 2^{-2i+1} =: \hat{C}^u_i \quad \mbox{and} \quad \hat{C}^u_{i+1} \leq \frac{1}{4} \hat{C}^u_i.
  \end{equation*}
  Clearly, $\hat{C}^u_1 \leq \sum_{i=1}^{n_\Achannel} \hat{C}^u_i \leq 2 \hat{C}^u_1$ due to the convergence of the geometric series. In other words:
  \begin{equation*}
    \Pr(B^u) \leq 2 C^u_1 = \bigO(\pi_\ell \activity(u)\AAC(u)).
  \end{equation*}
  
  % Since $B^u=H_u$, this 
  This
  concludes the proof of the first part of the claim, equations (\ref{eq:claimequationsupper}). Note that in both cases $\AAC(u) \leq 2$ and $\AAC(u) > 2$ we had that
  \begin{equation}
    \label{eq:BulambdaUB}
    \Pr(B^u_\lambda)=\Omega(B^u).
  \end{equation}
  % Note that $\Pr(D^u) \leq \Pr(B^u)$. \sebastian{why did i put this here??}


  % \sebastian{ANCHOR; the changes to the definition of $D^u$ must be incorporated here. For $\AAC(u) > 2$ and $m=0$ it should be possible to show that no node in any constant neighborhood is on channel $\Achannel_\lambda$ with constant probability. For $m\geq 1$ we should be able to show that any node $x$ with high $\AAC(x)$ has collisions with probability arbitrarily close to $1$ (depending on $\pi_\ell$). The case $\AAC(u) \leq 2$ has not yet been looked at.}

  \vspace{3mm}
  \paraclose{Lower Bounds}
  \\
  For lower bounds we study 2 specific channels, depending whether $\AAC(u)$ is greater than $2$ or not. More precisely, we study $\Achannel_\lambda$, where $\lambda := \max\set{1, \log \AAC(u)}$ and show that event $D^u$ happens on this channel with the desired probability. 
  The base idea is to show that \wcp no node $x \in N^3_\Astate(u)$ with $\AAC(x) \hide{\lessapprox} \lesssim \AAC(u)$ is listening on channel $\Achannel_\lambda$ at all, while all nodes $x$ with $\AAC(x) \hide{\gtrapprox}\gtrsim \AAC(u)$ experience a collision on $\Achannel_\lambda$.

  \paraclose{Case 1: \boldmath{$\AAC(u) > 2$, $\lambda = \log \AAC(u)$ and $2^{-\lambda} = 1/\AAC(u)$}}.

  % First, let $\AAC(u) > 2$, i.e., $\lambda = \log \AAC(u)$ and $2^{-\lambda} = 1/\AAC(u)$.
  % First we look at the events $B^{u,v}$, as above, starting like in (\ref{eq:BuviUB}).

  We start with some definitions. We define 
  $$X^{u,v}_m := \set{x \in N^3_\Astate(v)\setminus\set{u,v}: 10m \AAC(u) \leq \AAC(x) < 10(m+1) \AAC(u)}.$$ 
  Let $F^{u,v}_{\lambda,m}$ be the event that \emph{no} $x \in X^{u,v}_m$ receives \emph{any} message broadcasted  on $\Achannel_\lambda$ and let $E^x_\lambda$ be the event that $x \in \Astate$ \emph{successfully} receives a message on channel $\Achannel_\lambda$. If $x \in N_\Astate(v)\setminus\set{u}$, then $E^x_\lambda|B^{u,v}_\lambda$ implies that $x$ receives $v$'s message.
  % Let $q_\lambda^w$ be the probability that node $w$ does broadcast on channel $\Achannel_\lambda$, i.e., $q_\lambda^w = (1-\pi_\ell)\activity(w)2^{-\lambda} \leq 1/4$, and accordingly $\bar{q}^w_\lambda := 1-q^w_\lambda \geq 3/4$. 
  % We use multiple times that $\prod_{w \in A\setminus B} \bar{q}^w_\lambda \leq \big(\frac{4}{3}\big)^{|B|} \prod_{w \in A} \bar{q}^w_\lambda$. 
  % We use $\mathbbm{1}_A(x)$ as the indicator function whether $x \in A$ or not, e.g., $\mathbbm{1}_{N_\Astate(v)}(x)$ evaluates to $1$ if $x \in N_\Astate(v)$.
  % , and let $q_i^w = 1$ if $w \notin N_\Astate(u)$. 
  Further, $p_\lambda^{u,v} = \pi_\ell(1-\pi_\ell)\activity(u)\activity(v)2^{-2\lambda}$ is the probability that nodes $u$ and $v$ meet on channel $\Achannel_\lambda$ with $u$ listening and $v$ broadcasting. 

  % Let $x$ be a node in $N^3_\Astate(v)$.
  Apparently,
  \begin{equation}
    \label{eq:3}
    \Pr(B_\lambda^{u,v})
    =
    p_\lambda^{u,v} \prod_{w \in N_\Astate(u) \setminus\set{v}} \bar{q}_\lambda^w.
  \end{equation}
  We want to calculate $\Pr(E^x_\lambda|B^{u,v}_\lambda)$. For that we need to distinguish between the two cases $x \in N_\Astate(v)\setminus\set{u}$ and $x \notin N^1_\Astate(v)$. For the first case, no other neighbor of $x$ than $v$ is allowed to broadcast, while in the second case exactly one neighbor of $x$ needs to broadcast on $\Achannel_\lambda$.

  % \begin{equation}
  \begin{multline}
    x \in N_\Astate(v)\setminus\set{u}: 
    \quad
    \Pr(E^x_\lambda|B^{u,v}_\lambda) 
    = 
    \frac{\Pr(B^{u,v}_\lambda \cap E^x_\lambda)}{\Pr(B^{u,v}_\lambda)} 
    \\
    =
    \frac{1}{\Pr(B^{u,v}_\lambda)} \frac{\Pr(B^{u,v}_\lambda)}{\bar{q}^x_\lambda}  \pi_\ell\activity(x) 2^{-\lambda}\prod_{y \in  N_\Astate(x)\setminus\set{u,v}} \bar{q}_\lambda^y
    % =
    % \frac{\Pr(B^{u,v}_\lambda)}{\bar{q}^x_\lambda} \frac{\pi_\ell\activity(x) 2^{-\lambda}}{\Pr(B^{u,v}_\lambda)} \prod_{y \in  N_\Astate(x)\setminus\set{u,v}} \bar{q}_\lambda^y
    \leq
    \frac{4}{3} \pi_\ell \frac{\activity(x)}{\AAC(u)} \prod_{y \in N_\Astate(x)\setminus\set{u,v}} \bar{q}_\lambda^y
    \label{eq:lb1}
  \end{multline}
  % \end{equation}

  \begin{multline}
    x \notin N^1_\Astate(v):
    \quad
    \Pr(E^x_\lambda|B^{u,v}_\lambda) 
    =
    \Pr(E^x_\lambda|u \text{ listens}) 
    % \\ 
    =
    \pi_\ell \activity(x) 2^{-\lambda} \cdot \sumleft{y \in N_\Astate(x)\setminus\set{u}}{
      % (1-\pi_\ell)\activity(y)2^{-\lambda}
      q^y_\lambda
    } \cdot \prodleft{z \in N_\Astate(x)\setminus\set{u,y}}{
      % (1-(1-\pi_\ell)\activity(z)2^{-\lambda})
      \bar{q}^z_\lambda
    }
    \\
    =
    \pi_\ell \activity(x) 2^{-\lambda} \cdot \sumleft{y \in N_\Astate(x)\setminus\set{u}}{
      % \overbrace{(1-\pi_\ell)}^{\leq 1}
      (1-\pi_\ell)
      \activity(y)
      % \overbrace{2^{-\lambda}}^{=\AAC(u)}
      2^{-\lambda}
      % q^y_\lambda
    } \cdot \prodleft{z \in N_\Astate(x)\setminus\set{u,y}}{
      % (1-(1-\pi_\ell)\activity(z)2^{-\lambda})
      \bar{q}^z_\lambda
    }
    % 
    % \stackrel{(*)}{\leq}
    \leq
    \pi_\ell\frac{\activity(x)}{\AAC(u)} \cdot \frac{\AAC(x)}{\AAC(u)} \prodleft{z \in N_\Astate(x)\setminus\set{u,y}}{\bar{q}^z_\lambda}
    % =
    % \frac{\Pr(B^{u,v}_\lambda)}{\bar{q}^x_\lambda} \frac{\pi_\ell\activity(x) 2^{-\lambda}}{\Pr(B^{u,v}_\lambda)} \prod_{y \in  N_\Astate(x)\setminus\set{u,v}} \bar{q}_\lambda^y
    % \leq
    % \frac{4}{3} \pi_\ell \activity(x) 2^{-\lambda} \prod_{y \in N_\Astate(x)\setminus\set{u,v}} \bar{q}_\lambda^y
    \label{eq:lb2}
  \end{multline}
  \hide{
    $(*)$ follows from the fact that 
    $$\sum_{y \in N_\Astate(x)\setminus\set{u,v}}q^y_\lambda 
    = 
    \sumleft{y \in N_\Astate(x)\setminus\set{u,v}}{(1-\pi_\ell)\activity(y)2^{-\lambda}}
    \leq 
    \frac{\AAC(x)}{\AAC(u)}.
    $$
  }
  
  \hide{
    For $x \in N_\Astate^3(v)\setminus N_\Astate^1(v)$ we get a similar result:
    \begin{eqnarray*}
      % \Pr(B_i^{u,v}) 
      % &=& 
      % p_i^{u,v} \bar{q}_i^x \prod_{w \in N_\Astate(u) \setminus\set{v,x}} \bar{q}_i^w,
      % \\
      \Pr(E_\lambda^x \cap B_\lambda^{u,v}) 
      &=& 
      \Pr(B_\lambda^{u,v}) \pi_\ell \activity(x) 2^{-\lambda} \cdot \sumleft{y \in N_\Astate(x)\setminus\set{u,v}}{(1-\pi_\ell)\activity(y)2^{-\lambda}} \cdot \underbrace{\prodleft{z \in N_\Astate(x)\setminus\set{u,y}}{(1-(1-\pi_\ell)\activity(z)2^{-\lambda})}}_{\leq 1}
      \\
      &\leq&
      \Pr(B_\lambda^{u,v}) \pi_\ell \activity(x) 2^{-\lambda} (1-\pi_\ell)2^{-\lambda}\AAC(x) \leq \Pr(B_\lambda^{u,v}) \pi_\ell \activity(x) 2^{-2\lambda} \AAC(x)
      % , \text{ and}
      \\
      \Pr(E_\lambda^x|B_\lambda^{u,v}) 
      &\leq& 
      \pi_\ell \activity(x) 2^{-2\lambda} \AAC(x)
      \stackrel{\AAC(x) \leq 10 \AAC(u)}{\leq}
      10 \pi_\ell \activity(x) 2^{-\lambda}
    \end{eqnarray*}
  }

  
  % Thus, for any $x \in X^{u,v}_0$, $\Pr(E_\lambda^x|B_\lambda^{u,v}) \leq    10 \pi_\ell \activity(x) 2^{-\lambda}$.
  
  % This is at most $\frac{4}{3}\pi_\ell \activity(x) 2^{-\lambda}$ and therefore  $\Pr(E_\lambda^x|B_\lambda^{u,v}) \leq  \frac{4}{3}\pi_\ell \activity(x) 2^{-\lambda}$ for any $x\in N_\Astate^3(v)$.
  % \sebastian{not true. here we have $2^{-2i}\AAC(x)$, not $2^{-2i}\AAC(u)$}

  
  % Let $x \in X^{u,v}_0$, then we upper bound $\Pr(E^x_i|B^{u,v}_i)$ with the probability that $x$ visits channel $\Achannel_i$ and chooses to listen. At first assume that $x \notin N(u)$. Then:
  % % Note that if $x \in N(u)$, then conditioning on $B^{u,v}_i$ makes it much less likely for $x$ to be on channel $\Achannel_i$, more precisely, the probability goes down
  % \begin{equation}
  %   \Pr(E^x_i|B^{u,v}_i) \leq \pi_\ell \activity(x) 2^{-i}
  % \end{equation}
  % If $x \in N(u)$, however, then event $B^{u,v}_i$ already implies that $x$ is listening and we upper bound with the probability that $x$ visits channel $\Achannel_i$: $\activity(x) 2^{-i}$. Conditioning on $B^{u,v}_i$, however, reduces the likeliness of $x$ to be on channel $\Achannel_i$ by a factor of $\pi_\ell$ and therefore, regardless whether $x \in N(u)$ or $x \notin N(u)$, 
  % \begin{equation}
  %   \Pr(E^x_i|B^{u,v}_i) \leq \pi_\ell \activity(x) 2^{-i}
  % \end{equation}

  Now, using Lemma \ref{lemma:weightedturan}, observe that $\sum_{x \in N^3(u)} \frac{\activity(x)}{\Activity(x)} \leq \alpha^3$ and therefore:
  \begin{equation}
    \label{eq:weightedturanAAC}
    \sum_{x \in X^{u,v}_m} \activity(x) 
    = \sum_{x \in X^{u,v}_m} \frac{\activity(x)}{\Activity(x)} \Activity(x) 
    \leq \sum_{x \in X^{u,v}_m} \frac{\activity(x)}{\Activity(x)} \BB{\AAC(x) + \frac{1}{2}}
    \leq 10(m+1)\alpha^3\AAC(u) + \alpha^3 
    % \stackrel{\AAC(u)>1}{\leq} 11\alpha^3\AAC(u)
  \end{equation}
  
  We first look at the case $m=0$. 

  \paraclose{Case 1a: \boldmath{$\AAC(u) > 2$, $m=0$.}}
  Then, by (\ref{eq:weightedturanAAC}), $\sum_{x \in X^{u,v}_m} \activity(x) \leq 11\alpha^3\AAC(u)$. 
  Also, (\ref{eq:lb1}) can be upper bounded by $\frac{4}{3}\pi_\ell \frac{\activity(x)}{\AAC(u)}$ (since $\bar{q}^y_\lambda \leq 1$). 
  For (\ref{eq:lb2}) we note that $\AAC(x)\leq 10\AAC(u)$ and get combined that $\Pr(E^x_\lambda|B^{u,v}_\lambda) \leq 10\pi_\ell \frac{\activity(x)}{\AAC(u)}$, regardless whether $x \in N^1_\Astate(v)$ or not.
  
  
  % Combining everything we have, we get
  
  % Thus,
  \begin{equation*}
    \Pr(F^{u,v}_{\lambda,0}|B^{u,v}_\lambda)
    \geq \prod_{x \in X^{u,v}_0} \brackets{1- 10\pi_\ell \frac{\activity(x)}{\AAC(u)}}
    \geq e^{-2\frac{10\pi_\ell}{\AAC(x)}\sum_{x\in X^{u,v}_0}\activity(x)} 
    \stackrel{(\ref{eq:weightedturanAAC})}{\geq} e^{-220\alpha^3\pi_\ell} 
    \stackrel{\pi_\ell \leq \frac{1}{2}}{=}
    \Omega(1).
  \end{equation*}
  % For $\AAC(u) >2$ and channel 
  % With $i=\lambda := \log \AAC(u)$ this is in $\Omega(1)$. 

  \paraclose{Case 1b: \boldmath{$\AAC(u) > 2$, $m\geq 1$.}}
  % Let now $m\geq 1$. 
  We show that, \wcp, all $x \in \bigcup_{m\geq 1} X^{u,v}_m$, that listen on channel $\Achannel_\lambda$, have a collision.
  % Again via Lemma \ref{lemma:weightedturan} we get that $\sum_{x \in X^{u,v}_m} \activity(x) \leq (10(m+1)\AAC(u)+\frac{1}{2})\alpha^3 \leq 11(m+1)\alpha^3\AAC(u)$. 
  % Note that inequality (\ref{eq:weightedturanAAC}) does also hold for $m \geq 1$.
  For $E^x_\lambda$ to happen, exactly one of $x$'s neighbors has to broadcast. We look again first at $x \in N_\Astate(v)\setminus\set{u}$. We plug in the values for $\bar{q}^y_\lambda$ into (\ref{eq:lb1}) and we use that $\AAC(x)\geq 10m\AAC(u)$ to get
  
  \begin{equation*}
    % \begin{eqnarray*}
    \Pr(E^x_\lambda|B^{u,v}_\lambda) 
    % &\leq&
    \leq 
    \frac{4}{3}\pi_\ell \frac{\activity(x)}{\AAC(u)} 
    % \prodleft{y \in N_\Astate(x)\setminus\set{u,v}}{\bigbrackets{ 1-(1-\pi_\ell)\frac{\activity(y)}{\AAC(u)}}}
    \prod_{y \in N_\Astate(x)\setminus\set{u,v}} \Big( 1-(1-\pi_\ell)\frac{\activity(y)}{\AAC(u)}\Big)
    \leq 
    \frac{64}{27}\pi_\ell \frac{\activity(x)}{\AAC(u)} e^{-\frac{1}{2}\frac{\AAC(x)}{\AAC(u)}}
    \leq
    3\pi_\ell \frac{\activity(x)}{\AAC(u)} e^{-5m}
    % \end{eqnarray*}
  \end{equation*}
  For $x \in N_\Astate^3(v)\setminus N_\Astate^1(v)$ we do the same with (\ref{eq:lb2}) and also use that $\AAC(x) \leq 10(m+1)\AAC(u)$:

  % \begin{equation*}
  %   \begin{multline}
  \begin{eqnarray*}
    \Pr(E^x_\lambda|B^{u,v}_\lambda) 
    &\leq&
    % \pi_\ell\frac{\activity(x)}{\AAC(u)} \cdot \frac{\AAC(x)}{\AAC(u)} \prodleft{z \in N_\Astate(x)\setminus\set{u,y}}{\bigbrackets{ 1-(1-\pi_\ell)\frac{\activity(z)}{\AAC(u)}}}
    \pi_\ell\frac{\activity(x)}{\AAC(u)} \cdot \frac{\AAC(x)}{\AAC(u)} \prod_{z \in N_\Astate(x)\setminus\set{u,y}} \Big(1-(1-\pi_\ell)\frac{\activity(z)}{\AAC(u)}\Big)
    \\ &\leq& 
    % \leq
    \frac{16}{9}10(m+1)\pi_\ell\frac{\activity(x)}{\AAC(u)}e^{-\frac{1}{2}\frac{\AAC(x)}{\AAC(u)}}
    % \\ &\leq& 
    \leq
    40m\pi_\ell \frac{\activity(x)}{\AAC(u)} e^{-5m}
  \end{eqnarray*}
  % \end{multline}
  % \end{equation*}


  % \sebastian{ANCHOR. note to myself: here we have $\AAC(x)$ together with $2^{-2i}$, so with $i=\lambda$, this does not trivially lead to the result where $x \in N(v)$}

  % The fraction $\frac{16}{9}$ stems from the fact that in the product over all $z$ we do not include $u$ and $y$, in $\AAC(x)$, which we use in our upper bound, those values are included, though. At most the product in question decreases by a factor of $3/4$ for each node.

  For all $x \in X^{u,v}_m$ we therefore have $\Pr(E_\lambda^x|B_\lambda^{u,v})  \leq 40m\pi_\ell \frac{\activity(x)}{\AAC(u)} e^{-5m}$. Recall that by (\ref{eq:weightedturanAAC}) we can upper bound $\sum_{x \in X^{u,v}_m} \activity(x)$ by $22m\alpha^3\AAC(u)$.

  
  % If we choose $i=\lambda=\log \AAC(u)$ and recall that $\AAC(x)\geq 10m\AAC(u)$, we get
  \hide{
    \begin{equation}
      \Pr(E^x_\lambda|B^{u,v}_\lambda) 
      \leq \frac{16}{3}\pi_\ell \frac{\activity(x)}{\AAC(u)} e^{-\frac{\AAC(x)}{2\AAC(u)}}
      % \stackrel{\AAC(x)\geq 10m\AAC(u)}{\leq} 
      \leq
      \frac{16}{3}\pi_\ell \frac{\activity(x)}{\AAC(u)} e^{-5m}
    \end{equation}
  }
  For $F^{u,v}_{\lambda,m\geq 1} := \bigcap_{m\geq 1}F^{u,v}_{\lambda,m}$ we get
  \begin{eqnarray*}
    % \label{eq:}
    \Pr(F^{u,v}_{\lambda, m\geq 1}|B^{u,v}_\lambda) 
    &\geq& 
    \prod_{m\geq 1} \prod_{x \in X^{u,v}_m} (1-\Pr(E^x_\lambda|B^{u,v}_\lambda))
    \geq
    \prod_{m\geq 1} \prod_{x \in X^{u,v}_m} \Big(1-40m\pi_\ell \frac{\activity(x)}{\AAC(u)} e^{-5m}\Big)
    % \stackrel{}{\geq}
    \\
    &\geq& 
    % \geq 
    \prod_{m\geq 1} e^{-80m\pi_\ell e^{-5m}\sum_{x \in X^{u,v}_m} \frac{\activity(x)}{\AAC(u)}}
    % \\
    % &\geq& 
    \geq
    \prod_{m\geq 1} e^{-1760\pi_\ell \alpha^3  m^2 e^{-5m}}
    % \\
    % &\geq&
    \geq 
    e^{ -1760\pi_\ell\alpha^3 \sum_{m\geq 1}m^2e^{-5m} } 
    \\
    &\geq& 
    e^{-12\pi_\ell\alpha^3}
    =
    \Omega(1).
  \end{eqnarray*}
  
  Let us now define $F^{u,v}_\lambda$ as $F^{u,v}_{\lambda,m=0} \cap F^{u,v}_{\lambda,m\geq 1}$, then we get:
  % With this we calculate $\Pr(D^{u,v}_\lambda$:
  \begin{equation*}
    \Pr(D^{u,v}_\lambda) = \Pr(B^{u,v}_\lambda \cap F^{u,v}_\lambda)
    = \Pr(B^{u,v}_\lambda) \Pr(F^{u,v}_{\lambda,m=0}|B^{u,v}_\lambda) \Pr(F^{u,v}_{\lambda,m\geq 1}|B^{u,v}_\lambda) = \Omega(\Pr(B^{u,v}_\lambda))
  \end{equation*}
  With the results from above, this concludes the analysis for the case of $\AAC(u)>2$.

  \paraclose{Case 2: \boldmath{$\AAC(u) \leq 2$, $\lambda = 1$ and $2^{-\lambda} = 1/2$}}.

  % Thus, from now on, let $\AAC(u) \leq 2$ and therefore $\lambda := 1$.
  
  
  % For event $D^{u,v}_\lambda$ it holds that
  % $$D^{u,v}_\lambda = (\Pr(B^{u,v}_\lambda \cap \Pr(F^{u,v}_{\lambda,m=0} \cap \Pr(F^{u,v}_{\lambda,m\geq 1}.$$
  % With $\Pr(B^{u,v}_\lambda) = \Omega(\pi_\ell \frac{\activity(u)}{\AAC(u)})$ and the results from above we get ...


  % This concludes our analysis for the case of $\AAC(u) > 2$. Thus, from now on, let $\AAC(u) \leq 2$. Thus, from now on, $\lambda = 1$.
  % Combining cases $m=0$ and $m\geq 1$ yields that if $u$ hears from $v$ on $\Achannel_i$, then \wcp\ no other node receives $v$'s message.


  % We next look at the case $\AAC(u) \leq 1$ before we 

  For this case we redefine $X^{u,v}_m := \set{x \in N^3_\Astate(v)\setminus\set{u,v}: 10m \leq \AAC(x) < 10(m+1)}$. 
  Analogously to (\ref{eq:lb1}) and (\ref{eq:lb2}) we get (with $2^{-\lambda}=1/2$):


  \begin{eqnarray}
    x \in N_\Astate(v)\setminus\set{u}: 
    &\quad&
    \Pr(E^x_\lambda|B^{u,v}_\lambda) 
    =
    \Pr(E^x_1|B^{u,v}_1) 
    \leq 
    \frac{2}{3}\pi_\ell \activity(x) \prod_{y \in N_\Astate(x)\setminus\set{u,v}} \bar{q}_\lambda^y
    \label{eq:lb3}
    \\
    x \notin N^1_\Astate(v):
    &\quad&
    \Pr(E^x_\lambda|B^{u,v}_\lambda) 
    =
    \Pr(E^x_1|B^{u,v}_1) 
    \leq
    \frac{\pi_\ell}{4}\activity(x) \AAC(x) \prodleft{z \in N_\Astate(x)\setminus\set{u,y}}{\bar{q}^z_\lambda}
    \label{eq:lb4}
  \end{eqnarray}


  Like with (\ref{eq:weightedturanAAC}), Lemma \ref{lemma:weightedturan} gives us that 
  \begin{equation}
    \label{eq:weightedturanAAC2}
    \sum_{x \in X^{u,v}_m} \activity(x) \leq 10(m+1)\alpha^3+\frac{1}{2}\alpha^3 \leq 11(m+1)\alpha^3.
  \end{equation}
  \paraclose{Case 2a: \boldmath{$\AAC(u) \leq 2$, $m=0$.}}
  
  From \ref{eq:weightedturanAAC2} we get $\sum_{x \in X^{u,v}_0} \activity(x) \leq 11\alpha^3$. With $\bar{q}^y_\lambda = \bar{q}^y_1 \leq 1$ and $\AAC(x) \leq 10$ we get for all $x \in X^{u,v}_0$ that $\Pr(E^x_\lambda|B^{u,v}_\lambda) = \Pr(E^x_1|B^{u,v}_1) \leq 3\pi_\ell \activity(x)$.
  % We start with $x \in N_\Astate(v)\setminus\set{u}$. 

  Thus,
  \begin{equation*}
    \Pr(F^{u,v}_{\lambda,0}|B^{u,v}_\lambda) 
    \geq \prod_{x \in X^{u,v}_0} (1- 3\pi_\ell \activity(x)) 
    \geq e^{-66\pi_\ell\alpha^3 } = \Omega(1)
  \end{equation*}
  % For $i=1$ this is in $\Omega(1)$. 

  \paraclose{Case 2b: \boldmath{$\AAC(u) \leq 2$, $m\geq 1$.}}
  Note that since $\lambda=1$ we have $q^w_1 = (1-\pi_\ell)\activity(w)2^{-\lambda} \geq \activity(w)/4$ and therefore $\bar{q}^w_1 \leq e^{-\activity(w)/4}$. We use (\ref{eq:lb3}) and (\ref{eq:lb4}) to show that for \emph{any} $x \in X^{u,v}_m$

  \begin{equation*}
    \Pr(E^x_\lambda|B^{u,v}_\lambda) \leq \frac{1}{4} \pi_\ell \activity(x) 20m \Bigbrackets{\frac{4}{3}}^2\prodleft{z \in N_\Astate(x)}{\bar{q}^z_\lambda}
    \leq
    10m \pi_\ell \activity(x) e^{-2.5m}
  \end{equation*}

  As indicated by (\ref{eq:weightedturanAAC2}), $\sum_{x \in X^{u,v}_m} \activity(x) \leq 22m\alpha^3$ for $m\geq 1$.
  For $F^{u,v}_{\lambda,m\geq 1} = \bigcap_{m\geq 1}F^{u,v}_{1,m}$ we thus get again
  \begin{eqnarray*}
    % \label{eq:}
    \Pr(F^{u,v}_{1, m\geq 1}|B^{u,v}_1) 
    &\geq& 
    \prod_{m\geq 1} \prod_{x \in X^{u,v}_m} (1-\Pr(E^x_1|B^{u,v}_1))
    \geq
    \prod_{m\geq 1} \prod_{x \in X^{u,v}_m} \bigbrackets{ 1-10m\pi_\ell \activity(x) e^{-2.5m} }
    % \stackrel{}{\geq}
    \\
    &\geq& 
    % \geq 
    \prod_{m\geq 1} e^{-20m\pi_\ell e^{-2.5m}\sum_{x \in X^{u,v}_m} \activity(x)}
    % \\
    % &\geq& 
    \geq
    \prod_{m\geq 1} e^{-440m\pi_\ell \alpha^3 e^{-5m}}
    % \\
    % &\geq&
    \geq 
    e^{ -440\pi_\ell\alpha^3 \sum_{m\geq 1}me^{-2.5m} } 
    \\
    &\geq& 
    e^{-50\pi_\ell\alpha^3}
    =
    \Omega(1).
  \end{eqnarray*}

  Completely analogously to the case $\AAC(x)>2$ it holds that $\Pr(D^{u,v}_1) = \Omega(\Pr(B^{u,v}_1))$.

  % \sebastian{what about the other channels in the case $\AAC(u)<2$? it's unlikely that anything happens there, but how do we express this in a short way?}

  % \vspace{4mm}\sebastian{ANCHOR}\vspace{4mm}

  % \sebastian{we still need to combine the $D^{u,v}_i$ results to $D^u_i$ and then $D^u$.}

  Let $c$ be the constant such that $\Pr(D^{u,v}_\lambda) \geq c \Pr(B^{u,v}_\lambda)$ for any $v \in N_\Astate(u)$. Then, since $D^u_\lambda = \bigdotcup_{v \in N_\Astate(v)} D^{u,v}_\lambda$ and $B^u_\lambda = \bigdotcup_{v \in N_\Astate(v)} B^{u,v}_\lambda$, it most hold that $\Pr(D^u_\lambda) \geq c \Pr(B^u_\lambda)$.
  Also, $\Pr(D^u) \geq \Pr(D^u_\lambda)$ and since by (\ref{eq:BulambdaUB}) $\Pr(B^u_\lambda)=\Omega(\Pr(B^u))$, we get that $\Pr(D^u)=\Omega(\Pr(B^u))$.

  \hide{
    We now focus on events $B^{u,v}_i$. Similar to previous calculations we get.
    \begin{equation}
      \label{eq:BuviLB}
      \Pr(B^{u,v}_i) 
      \geq \frac{1}{2}\pi_\ell \activity(u)\activity(v)2^{-2i} e^{-2\AAC(u)2^{-i}}
    \end{equation}
    Event $D^{u,v}_\lambda$ is the happening of both events $B^{u,v}_\lambda$ and $F^{u,v}_\lambda$. Let $\AAC(u) > 2$, then
    \begin{equation}
      \Pr(D^{u,v}_\lambda) = \Pr(B^{u,v}_\lambda) \Pr(F^{u,v}_\lambda | B^{u,v}_\lambda)
      = \Omega(\pi_\ell \frac{\activity(u)}{\AAC(u)}).
    \end{equation}
    For $\AAC(u) \leq 2$ we similarly get
    \begin{equation}
      \Pr(D^{u,v}_\lambda) = \Pr(D^{u,v}_1) = \Omega(\pi_\ell \activity(u)\AAC(u)).
    \end{equation}
  }

  This finishes the proof for the second part of the claim, equations (\ref{eq:claimequationslower})
\end{proof}




% =====================
% old write-up
\hide{
  \begin{lemma}
    \label{lemma:heraldwcpgoodherald}
    Let $B(r)^{u,v}$ be the event that in round $r$ node $u \in \Astate_r$ receives a message from one of its neighbors $v\in \Astate_{r-1}$, neither of them neighboring any leader, herald or herald candidate, and let $\hat H(r')^{u',v'}$ be the event that at the beginning of round $r'$ node $u' \in \Hstate_{r'-1}$ and $v' \in \Lstate_{r'-1}$ form a good \lhp. Then
    \begin{equation}
      % \label{eq:4}
      \Pr(\hat H(r+8)^{u,v}|B(r)^{u,v}) = \Omega(1)
    \end{equation}
  \end{lemma}

  \sebastian{notes for later: we also don't want herald candidates in a broader neighborhood. leaders and heralds, however, must be allowed to exist nearby. Thus, statement needs to be extended such that fabian's proof does fit.}
  % \sebastian{this really needs to be checked for errors; as it must hold for any kind of scenario in which $u$ and $v$ are active in round $t$. e.g., this is wrong if they are neighboring another good leader-herald pair but manage to bypass their really low activity levels. i.e., we need to add a ton of additional requirements.}
  \sebastian{note for next adjustment: hinder that nodes communicate on channel $\lambda$ also in a larger radius around $u$.}


  % \begin{proof}
  The proof for the lemma is not straightforward. We consider the two cases of $\Activity(u)>2$ and $\Activity(u) \leq 2$ and for those we establish claims about the probabilities for $u$ to become a herald in general and a good herald in detail before we provide the proof for Lemma \ref{lemma:heraldwcpgoodherald}.
  Denote with $\Activity_\Astate(u)$ the activity mass of all active nodes in $N^1(u)$ and with $\AAC(u)$ the mass of those in $N(u)$, i.e., $\AAC(u)=\Activity_\Astate(u)-\activity(u)$.     


  \begin{claim}
    \label{claim:heraldbounds}
    Let $t$ be a round in which node $u$ is in state \Astate and $N_\Astate(u) \neq \emptyset$.
    % and $\Activity(u) \geq 1$.
    % , and in which it has a neighbor in the \hfilter. 
    Let $B^u$ be the event that in round $t$, $u$ moves to state
    $\Hstate'$ due to receiving a message from some node $v \in
    N_\Astate(u)$ on some channel $\Achannel_{\bar{lambda}}$. Further, let $D^u\subseteq B^u$ be the event that
    $B^u$ holds and no other node $v' \in N^3(v)\setminus\set{u}$
    % moves to one of the states $\Hstate'$ or $\Lstate'$, then
    receives any message on channel $\Achannel_{\bar{\lambda}}$ in round $t$. 
    \sebastian{this has been extended; $D^u$ previously only said that no node $v' \in N(v)$ gets the message from $v$.}
    It holds that
    \begin{eqnarray}
      \label{eq:claimequationsupper}
      \Pr(B^u) &=&
      \begin{cases}
        \bigO\brackets{\pi_\ell \frac{\activity(u)}{\AAC(u)}} & \AAC(u) > 2 \\
        \bigO\brackets{\pi_\ell \activity(u) \AAC(u)} & \AAC(u) \leq 2      
        % \bigO\brackets{\pi_\ell \frac{\activity(u)}{\Activity(u)}} & \AAC(u) > 1 \\
        % \bigO\brackets{\pi_\ell \activity(u) \Activity(u)} & \AAC(u) \leq 1      
      \end{cases},
      \\
      \label{eq:claimequationslower}
      \Pr(D^u) &=&
      \begin{cases}
        \Omega\brackets{\pi_\ell \frac{\activity(u)}{\AAC(u)}} & \AAC(u) > 2 \\
        \Omega\brackets{\pi_\ell \activity(u) \AAC(u)} & \AAC(u) \leq 2      
        % \Omega\brackets{\pi_\ell \frac{\activity(u)}{\Activity(u)}} & \AAC(u) > 1 \\
        % \Omega\brackets{\pi_\ell \activity(u) \Activity(u)} & \AAC(u) \leq 1      
      \end{cases}.
    \end{eqnarray}
    % \sebastian{all the values $\Activity(u)$ maybe need to be replaced by $\AAC(u)$. Should (hopefully) not affect the final proof.}
  \end{claim}

  \hideproof{proof:claim:heraldbounds}{provide information}{
    \begin{proof}
      In the calculations below we make use of the following inequalities.
      \begin{eqnarray}
        \label{eq:basic}
        1-\pi_\ell &\geq& 1/2 \\
        1-x &\leq& e^{-x}, \quad \forall x \\
        1-x &\geq& e^{-2x}, \forall x \in [0,1/2]
      \end{eqnarray}

      If $\AAC(u) > 2$, for simplicity, we assume that $\log \AAC(u)$ is a positive integer. It becomes clear from the proof that for non-integer values 
      % $\log \AAC(u) \in (\lfloor \log \AAC(u)\rfloor, \lceil\log\AAC(u)\rceil)$ 
      an adaption is straightforward, but hard to read.

      We let $B^{u,v}_i$ be the event that an \emph{active} node $u$ receives a message from an \emph{active} node $v$ on channel $\Achannel_i$, i.e., $u$ listens and $v$ broadcasts on $\Achannel_i$, while no other node $w \in (N_\Astate(u))\setminus\set{v}$ broadcasts on $\Achannel_i$. For different $v$ these events are disjoint, and we can define $B^u_i := \bigcup_{v \in N_\Astate(u)} B^{u,v}_i$ and we see that $B^u = \bigcup_{i=1}^{n_\Achannel} B^u_i$.

      % More restrictive are the analogously defined events $D^{u,v}_i$, $D^u_i$, in which we also require that no node $x \in N(v)\setminus\set{u}$ receives $v$'s message. In that case, $D^u=\bigcup_{i=1}^{n_\Achannel} D^u_i$ is the event that nodes $u$ and $v$ engage in the handshake protocol next round, without other herald candidates trying to do this with $v$ as well.

      More restrictive are the analogously defined events $D^{u,v}_i$, $D^u_i$, in which we also require that no node $x \in N^3(v)\setminus\set{u}$ receives a message on channel $i$. In that case, $D^u=\bigcup_{i=1}^{n_\Achannel} D^u_i$ is the event that nodes $u$ and $v$ engage in the handshake protocol in the round after they met on some channel $\Achannel_{\bar{\lambda}}$, without other nodes nearby having received something on that same channel. In particular, no other herald candidates try to engage with $v$ in the handshake protocol.

      \sebastian{the upper bounds should be untouched by the change to the definition of $D^u$.}

      % Note that $H_u = B^u$ and $\hat{H}_u \subset D^u$.


      % for upper bounds we can calculate in a rather rough way, but we have to upper bound over all channels
      % for lower bounds we just have to look at \Achannel_1 or \Achannel_\lambda, but we have to exclude the possibility of other receivers around $v$
      \paraclose{Upper Bounds}
      \begin{equation}
        \begin{split}
          \label{eq:BuviUB}
          \Pr(B^{u,v}_i)
          & = \pi_\ell \activity(u) 2^{-i}(1-\pi_\ell) \activity(v) 2^{-i} \prod_{w \in N_\Astate(u)\setminus\set{v}} \bigbrackets{ 1-(1-\pi_\ell)\activity(w)2^{-i} } \\
          & \leq \pi_\ell \activity(u)\activity(v)2^{-2i}
          \underbrace{\frac{1}{1-(1-\pi_\ell)\activity(v)2^{-i}}}_{\leq 2} e^{-\frac{1}{2}\AAC(u)2^{-i}}
        \end{split}
      \end{equation}

      \begin{equation}
        \label{eq:BuiUB}
        \Pr(B^u_i) \leq \pi_\ell \activity(u) \AAC(u) 2^{-2i+1} e^{-\AAC(u)2^{-i-1}} = 8\pi_\ell \frac{\activity(u)}{\AAC(u)} (\AAC(u) 2^{-i-1})^2 e^{-\AAC(u)2^{-i-1}} =: C^u_i
        % \leq \pi_\ell \activity(u) \Activity_\Astate(u) 2^{-2i+2} e^{-\Activity_\Astate(u)2^{-i-1}}
      \end{equation}

      Consider the case $\AAC(u) >2$. 
      % and for simplicity let $\lambda:= \log \AAC(u)$ be an integer. 
      It holds that $x^2e^{-x}=\bigO(1)$, and by using $x=\AAC(u)2^{-i}$ we get that $C^u_i = \bigO(\pi_\ell \frac{\activity(u)}{\AAC(u)})$ for any fixed $i$. Furthermore:
      \begin{align}
        \frac{C_{i+1}^u}{C_i^u} &= \frac{1}{4}e^{\frac{1}{4}\AAC(u)2^{-i}} < \frac{1}{2} & \forall i &\geq \log \AAC(u)\\
        \frac{C_{i}^u}{C_{i+1}^u} &=  4e^{-\frac{1}{4}\AAC(u)2^{-i}} < \frac{1}{2} & \forall i &\leq \log \AAC(u) -4
      \end{align}
      Thus, all $C^u_i$ with channels $\Achannel_i$ outside the range $\Achannel_{\lambda-4}, \dots, \Achannel_\lambda$ can be upper bounded by those within the range using the geometric series. But those within that range are in $\bigO(C^u_\lambda)=\bigO(\pi_\ell \frac{\activity(u)}{\AAC(u)})$.
      In total we get:
      \begin{equation}
        \label{eq:BuUB}
        \Pr(B^u) = \bigO(\pi_\ell \frac{\activity(u)}{\AAC(u)})
      \end{equation}
      Now consider the case $\AAC(u) \leq 2$ and let $\lambda :=1$.
      \begin{equation}
        \Pr(B^u_i) \leq \pi_\ell \activity(u) \AAC(u) 2^{-2i+1} =: \hat C^u_i
      \end{equation}
      Clearly, $C^u_\lambda=C^u_1 \geq \sum_{i=2}^{n_\Achannel} C^u_i$ due to the convergence of the geometric series. In other words:
      \begin{equation}
        \Pr(B^u) = \bigO(\pi_\ell \activity(u)\AAC(u))
      \end{equation}
      
      % Since $B^u=H_u$, this 
      This
      concludes the proof of the first part of the claim, equations (\ref{eq:claimequationsupper}).
      % Note that $\Pr(D^u) \leq \Pr(B^u)$. \sebastian{why did i put this here??}


      \sebastian{ANCHOR; the changes to the definition of $D^u$ must be incorporated here. For $\AAC(u) > 2$ and $m=0$ it should be possible to show that no node in any constant neighborhood is on channel $\Achannel_\lambda$ with constant probability. For $m\geq 1$ we should be able to show that any node $x$ with high $\AAC(x)$ has collisions with probability arbitrarily close to $1$ (depending on $\pi_\ell$). The case $\AAC(u) \leq 2$ has not yet been looked at.}

      \vspace{3mm}
      \paraclose{Lower Bounds}
      \\
      For lower bounds we study 2 specific channels, depending whether $\AAC(u)$ is greater than $2$ or not. More precisely, we study $\Achannel_\lambda$, where $\lambda := \max\set{1, \log \AAC(u)}$. 
      % First we look at the events $B^{u,v}$, as above, starting like in (\ref{eq:BuviUB}).

      Let $E^x_i$ be the event that $x$ \emph{successfully} receives a message on channel $\Achannel_i$. If $x \in N_\Astate(v)\setminus\set{u}$, then $E^x_i|B^{u,v}_i$ implies that $x$ receives $v$'s message. First, let $\AAC(u) > 2$.\\
      Define $X^{u,v}_m := \set{x \in N_\Astate(v)\setminus\set{u}: 10m \AAC(u) \leq \AAC(x) < 10(m+1) \AAC(u)}$. Let $F^{u,v}_{i,m}$ be the event that \emph{no} $x \in X^{u,v}_m$ receives $v$'s message, broadcasted  on $\Achannel_i$. Let $q_i^w$ be the probability that some node $w \in N_\Astate(u)$ does \emph{not} broadcast on channel $\Achannel_i$, i.e., $q_i^w = 1-(1-\pi_\ell)\activity(w)2^{-i} \geq 3/4$, and let $q_i^w = 1$ if $w \notin N_\Astate(u)$. Further, $p_i^{u,v} = \pi_\ell(1-\pi_\ell)\activity(u)\activity(v)2^{-2i}$ is the probability that nodes $u$ and $v$ meet on channel $\Achannel_i$ with $u$ listening and $v$ broadcasting. Then
      \begin{eqnarray}
        \Pr(B_i^{u,v}) 
        &=& 
        p_i^{u,v} q_i^x \prod_{w \in N_\Astate(u) \setminus\set{v,x}} q_i^w,
        \\
        \Pr(E_i^x \cap B_i^{u,v}) 
        &=& 
        \frac{\Pr(B_i^{u,v})}{q_x} \pi_\ell \activity(x) 2^{-i}, \text{ and}
        \\
        \Pr(E_i^x|B_i^{u,v}) 
        &\leq& 
        \frac{4}{3} \pi_\ell \activity(x) 2^{-i}
      \end{eqnarray}

      % Let $x \in X^{u,v}_0$, then we upper bound $\Pr(E^x_i|B^{u,v}_i)$ with the probability that $x$ visits channel $\Achannel_i$ and chooses to listen. At first assume that $x \notin N(u)$. Then:
      % % Note that if $x \in N(u)$, then conditioning on $B^{u,v}_i$ makes it much less likely for $x$ to be on channel $\Achannel_i$, more precisely, the probability goes down
      % \begin{equation}
      %   \Pr(E^x_i|B^{u,v}_i) \leq \pi_\ell \activity(x) 2^{-i}
      % \end{equation}
      % If $x \in N(u)$, however, then event $B^{u,v}_i$ already implies that $x$ is listening and we upper bound with the probability that $x$ visits channel $\Achannel_i$: $\activity(x) 2^{-i}$. Conditioning on $B^{u,v}_i$, however, reduces the likeliness of $x$ to be on channel $\Achannel_i$ by a factor of $\pi_\ell$ and therefore, regardless whether $x \in N(u)$ or $x \notin N(u)$, 
      % \begin{equation}
      %   \Pr(E^x_i|B^{u,v}_i) \leq \pi_\ell \activity(x) 2^{-i}
      % \end{equation}

      Now, using Lemma \ref{lemma:weightedturan}, observe that $\sum_{x \in N^3(u)} \frac{\activity(x)}{\Activity(x)} \leq \alpha^3$ and therefore:
      \begin{equation}
        \label{eq:weightedturanAAC}
        \sum_{x \in X^{u,v}_0} \activity(x) 
        = \sum_{x \in X^{u,v}_0} \frac{\activity(x)}{\Activity(x)} \Activity(x) 
        \leq \sum_{x \in X^{u,v}_0} \frac{\activity(x)}{\Activity(x)} (\AAC(x) + \frac{1}{2})
        \leq 10(m+1)\alpha^3\AAC(u) + \alpha^3 
        % \stackrel{\AAC(u)>1}{\leq} 11\alpha^3\AAC(u)
      \end{equation}

      Thus,
      \begin{equation}
        \Pr(F^{u,v}_{i,0}|B^{u,v}_i)
        \geq \prod_{x \in X^{u,v}_0} (1- \frac{4}{3}\pi_\ell \activity(x) 2^{-i}) 
        \stackrel{\AAC(u)>1, \, m=0}{\geq} e^{-30\pi_\ell\alpha^3\AAC(u)2^{-i}}
      \end{equation}
      For $\AAC(u) >2$ and channel $\Achannel_\lambda = \Achannel_{\log \AAC(u)}$ this is in $\Omega(1)$. 

      Let now $m\geq 1$. We show that, \wcp, all $x \in \bigcup_{m\geq 1} X^{u,v}_m$, that listen on channel $\Achannel_\lambda$, have a collision.
      % Again via Lemma \ref{lemma:weightedturan} we get that $\sum_{x \in X^{u,v}_m} \activity(x) \leq (10(m+1)\AAC(u)+\frac{1}{2})\alpha^3 \leq 11(m+1)\alpha^3\AAC(u)$. 
      % Note that inequality (\ref{eq:weightedturanAAC}) does also hold for $m \geq 1$.
      For $E^x_i$ to happen, none of $x$'s neighbors other than $v$ may broadcast. Like before we get
      % We omit here to look at the cases $x \in N(u)$ and $x \notin N(u)$ separately, as above they yield the same results.
      \begin{equation}
        \Pr(E^x_i|B^{u,v}_i) 
        \leq \frac{4}{3}\pi_\ell \activity(x) 2^{-i} \prod_{y \in N_\Astate(x)\setminus\set{u,v}} \bigbrackets{ 1-(1-\pi_\ell)\activity(y)2^{-i} }
        \leq \frac{4}{3}\pi_\ell \activity(x) 2^{-i+2} e^{-\frac{1}{2}\AAC(x)2^{-i}}
      \end{equation}
      Choosing $i=\lambda=\log \AAC(u)$ results in 
      \begin{equation}
        \Pr(E^x_\lambda|B^{u,v}_\lambda) 
        \leq \frac{8}{3}\pi_\ell \frac{\activity(x)}{\AAC(u)} e^{-\frac{\AAC(x)}{2\AAC(u)}}
        \stackrel{\AAC(x)\geq 10m\AAC(u)}{\leq} 
        \frac{8}{3}\pi_\ell \frac{\activity(x)}{\AAC(u)} e^{-5m}
      \end{equation}
      For $F^{u,v}_{\lambda,m\geq 1} := \bigcap_{m\geq 1}F^{u,v}_{\lambda,m}$ we get
      \begin{equation}
        % \label{eq:}
        \Pr(F^{u,v}_{\lambda, m\geq 1}|B^{u,v}_\lambda) 
        \geq 
        \prod_{m\geq 1} \prod_{x \in X^{u,v}_m} \bigbrackets{ 1-\frac{8}{3}\pi_\ell \frac{\activity(x)}{\AAC(u)} e^{-5m} }
        \geq e^{ -30\pi_\ell \sum_{m\geq 1}(m+1)e^{-5m} } \geq e^{-\pi_\ell}
        =\Omega(1)
      \end{equation}
      % Combining cases $m=0$ and $m\geq 1$ yields that if $u$ hears from $v$ on $\Achannel_i$, then \wcp\ no other node receives $v$'s message.

      % We next look at the case $\AAC(u) \leq 1$ before we 

      For the case of $\AAC(u) \leq 2$ we redefine $X^{u,v}_m := \set{x \in N_\Astate(v)\setminus\set{u}: 10m \leq \AAC(x) < 10(m+1)}$. Again, we first look at $x \in X^{u,v}_0$ and get yet again
      \begin{equation}
        \Pr(E^x_i|B^{u,v}_i) \leq \frac{4}{3}\pi_\ell \activity(x) 2^{-i}
      \end{equation}
      Like with (\ref{eq:weightedturanAAC}), Lemma \ref{lemma:weightedturan} gives us that $\sum_{x \in X^{u,v}_m} \activity(x) \leq 10(m+1)\alpha^3+\frac{1}{2}\alpha^3 \leq 11(m+1)\alpha^3$. Thus,
      \begin{equation}
        \Pr(F^{u,v}_{i,0}|B^{u,v}_i) 
        \geq \prod_{x \in X^{u,v}_0} (1- \frac{4}{3}\pi_\ell \activity(x) 2^{-i}) 
        \geq e^{-30\pi_\ell\alpha^3 2^{-i}}
      \end{equation}
      For $i=1$ this is in $\Omega(1)$. Let $m\geq 1$, then
      \begin{equation}
        \Pr(E^x_1|B^{u,v}_1) 
        \leq \frac{4}{3}\pi_\ell \activity(x) e^{-\frac{\AAC(x)}{4}}
        \leq \frac{4}{3}\pi_\ell \activity(x) e^{-2.5m}
      \end{equation}
      For $F^{u,v}_{\lambda,m\geq 1} := \bigcap_{m\geq 1}F^{u,v}_{\lambda,m}$ we get
      \begin{equation}
        % \label{eq:}
        \Pr(F^{u,v}_{\lambda,m\geq 1}|B^{u,v}_\lambda) \geq \prod_{m\geq 1} \prod_{x \in X^{u,v}_m} \bigbrackets{ 1-\frac{4}{3}\pi_\ell \activity(x) e^{-2.5m} }
        \geq 
        e^{ -15\pi_\ell \sum_{m\geq 1}(m+1)e^{-2.5m} } \geq e^{-3\pi_\ell}
        =\Omega(1)
      \end{equation}

      Now, for both $\AAC \leq 2$ and $\AAC > 2$ a simple argument again combines the results for $m=0$ and $m\geq 1$ into 
      \begin{equation}
        \Pr(F^{u,v}_\lambda|B^{u,v}_\lambda) := \Pr(\bigcap_{m\geq 0}F^{u,v}_{\lambda,m}|B^{u,v}_\lambda) = \Omega(1).
      \end{equation}

      We now focus on events $B^{u,v}_i$. Similar to previous calculations we get.
      \begin{equation}
        \label{eq:BuviLB}
        \Pr(B^{u,v}_i) 
        \geq \frac{1}{2}\pi_\ell \activity(u)\activity(v)2^{-2i} e^{-2\AAC(u)2^{-i}}
      \end{equation}
      Event $D^{u,v}_\lambda$ is the happening of both events $B^{u,v}_\lambda$ and $F^{u,v}_\lambda$. Let $\AAC(u) > 2$, then
      \begin{equation}
        \Pr(D^{u,v}_\lambda) = \Pr(B^{u,v}_\lambda) \Pr(F^{u,v}_\lambda | B^{u,v}_\lambda)
        = \Omega(\pi_\ell \frac{\activity(u)}{\AAC(u)}).
      \end{equation}
      For $\AAC(u) \leq 2$ we similarly get
      \begin{equation}
        \Pr(D^{u,v}_\lambda) = \Pr(D^{u,v}_1) = \Omega(\pi_\ell \activity(u)\AAC(u)).
      \end{equation}
      This finishes the proof for the second part of the claim, equations (\ref{eq:claimequationslower})
    \end{proof}
  }

} % hide end




We are now ready to prove Lemma \ref{lemma:heraldwcpgoodherald}.

\begin{proof}[Proof of Lemma \ref{lemma:heraldwcpgoodherald}]
  According to Claim \ref{claim:heraldbounds}, since $D^u \subset B^u$, it holds that $\Pr(D^u|B^u) = \Omega(1)$. Thus, if $B(r)^{u,v}$ happens, where $u$ receives the message on channel $\Achannel_i$, then, \wcp, no other node $w' \in N^3(u)\setminus\set{u}$ (which includes $v$'s neighborhood) receives a message on $\Achannel_i$. If no other node $w' \in N^3(u)\setminus\set{u}$ receives a message on $\Achannel_i$, that means that all such nodes $w'$ either not operate on $\Achannel_i$, or, if they do, none or at least $2$ of their neighbors $w'' \in N^4(u)$ send a message on $\Achannel_i$. Using Lemma \ref{lemma:wcpnoherald}.(\ref{lemma:wcpnoherald:4}) by setting $k=4$, $\pi_\ell$ appropriately small and conditioning on the set $S=S^l \dcup S^b \dcup S^n$ of nodes as listening/broadcasting on channel $\Achannel_i$ or not operating on $\Achannel_i$ at all (denoted by event $Z:=\mathcal{S}^n_{\neg i} \wedge \mathcal{S}^b_i \wedge \mathcal{S}^l_i$), we get that $\Pr(H_{\neg i}|D^u)=\Pr(H_{\neg i}|Z) > 1/2$. 

  If in round $r$ both events $H_{\neg i}$ and $D^u$ happen (where $u$ gets its message on channel $\Achannel_i$), then in round $r+1$ nodes $u$ and $v$ meet on channel $\Hchannel$ and can perform the first round of the handshake protocol without any interruption from any other nearby nodes. By applying Lemma \ref{lemma:wcpnoherald}.(\ref{lemma:wcpnoherald:1}) multiple times, in rounds $r+1$ to $r+7$, \wcp, no other new herald is created in $N^3(u)$. Thus, \wcp, by the beginning of round $r+8$, $u$ and $v$ have emerged from the handshake as a good \lhp.
\end{proof}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../multichannel_mis_main"
%%% End: 

